Understanding and Improving Convolutional Neural Networks via Concatenated Rectified Linear Units

Recently, convolutional neural networks (CNNs) have been used as a powerful tool to solve many problems of machine learning and computer vision. In this paper, we aim to provide insight on the property of convolutional neural networks, as well as a generic method to improve the performance of many CNN architectures. Specifically, we first examine existing CNN models and observe an intriguing property that the filters in the lower layers form pairs (i.e., filters with opposite phase). Inspired by our observation, we propose a novel, simple yet effective activation scheme called concatenated ReLU (CRelu) and theoretically analyze its reconstruction property in CNNs. We integrate CRelu into several state-of-the-art CNN architectures and demonstrate improvement in their recognition performance on CIFAR-10/100 and ImageNet datasets with fewer trainable parameters. Our results suggest that better understanding of the properties of CNNs can lead to significant performance improvement with a simple modification.

==> Conclusion.tex <==
\cutsectionup
\section{Conclusion}
\label{sec:conclusion}
We propose a new activation scheme, $\cat$, which conserves both positive and negative linear responses after convolution so that each filter can efficiently represent its unique direction. 
%
%It is based on the premise that the lower layers of a standard deep CNN learns to disentangle the positive and negative phase after the linear convolution layer, which leads to producing pairs of highly correlated filters of  the opposite phase.
%
%
%Merely replacing $\relu$ with $\cat$ for the first few conv layers of an existing CNN architecture yields a substantial improvement in classification performance. 
%
%In addition, $\cat$ allows us to attain notable parameter reduction without sacrificing--if not boosting--classification performance when applied appropriately. 
%
%Following our experiments, we note that $\cat$ helps regularize model and extract more invariant features.
%
%More interestingly, contrary to common belief, even though the invariance scores of a deep CNN generally increase while going deeper, the progression is not strictly monotonic. 
%
%This discovery together with our earlier observation that $\cat$ achieves the most performance gain when integrating into \emph{the first few conv layers} casts light on the diverse functionality of convolution layers. 
%
%By not eliminating the negative phase information, $\cat$ allows for a better mathematical characterization of the reconstruction property of a CNN, an important indicator of how expressive and generalizable the corresponding CNN features are.
%
Our work demonstrates that $\cat$ improves deep networks with classification objective.
%
%Since $\cat$ draws power from preserving all the available information yet maintaining the non-saturated non-linearity at the same time, it can potentially benefit more complicated machine learning tasks such as structured output predication and image generation. 
Since $\cat$ preserves the available information from input while maintaining the non-saturated non-linearity, it can potentially benefit more complicated machine learning tasks such as structured output prediction and image generation. 
%
Another direction for future research involves engaging $\cat$ to the abundant set of existing deep neural network techniques and frameworks. %, such as replacing $\relu$ with Leaky $\relu$ and applying $\cat$ to recurrent neural networks.
%
We hope to investigate along these directions in the near future. 
%Indeed, a full range of possibilities that $\cat$ potentially enables is yet to be explored. 

%Our preliminary findings on the internal operation of existing CNN architectures sparked the idea of $\cat$. 
%
%The follow-up empirical experiments in turn confirmed our initial conjecture as well as brought new insights into the behavior of convolution layers. 
%
%The advancement of our studies conveys the message that by better understanding the nature of CNNs, we are able to reach their higher potential using only a simple architecture, a smaller number of parameters and a vanilla training procedure. 


==> CrossChannel.tex <==
\begin{table}[t]
\caption{\textbf{Correlation Comparison.} The averaged correlation between the normalized positive-negative-pair (pair) outgoing weights and the normalized unmatched-pair (non-pair) outgoing weights are both well below $1$ for all layers, indicating that the pair outgoing weights are capable of imposing diverse non-linear manipulation separately on the positive and negative components. \label{tab:correlation}}
\vspace{0.05in}
\centering
\small
\begin{tabular}{c|c|c} 
\hline
\multicolumn{3}{c}{ImageNet Conv1--7 $\cat$ Model}\\ \hline
layer & pair & non-pair \\ \hline
conv1 & 0.372 {\scriptsize$\pm 0.372$}  & 0.165 {\scriptsize$\pm 0.154$}   \\ \hline
conv2& 0.180 {\scriptsize$\pm 0.149$} & 0.157 {\scriptsize$\pm 0.137$}  \\ \hline 
conv3 & 0.462 {\scriptsize$\pm 0.249$} & 0.120 {\scriptsize$\pm 0.120$}   \\ \hline
conv4 & 0.175 {\scriptsize$\pm 0.146$}& 0.119  {\scriptsize$\pm 0.100$}   \\ \hline
conv5& 0.206 {\scriptsize$\pm 0.136$}& 0.105 {\scriptsize$\pm 0.093$}  \\ \hline 
conv6& 0.256 {\scriptsize$\pm 0.124$}& 0.086 {\scriptsize$\pm 0.080$}  \\ \hline 
conv7& 0.131 {\scriptsize$\pm 0.122$}& 0.080 {\scriptsize$\pm 0.070$}  \\ \hline 
\end{tabular}
\vspace{-0.15in}
\end{table}
\cutsectiondown

\cutsubsectionup
\subsection{Towards Learning Invariant Features}
\label{sec:invariant}
%
%Spatial pooling has been well researched from many perspectives~\cite{zeiler2013stochastic,lee2015generalizing}, but few endeavor to design effective cross-channel pooling since it is less trivial to define the pooling region.
%
%\citet{goodfellow2013maxout} studies the maxout nonlinearity that learns which channel to activate while zeroing out the other channels in the pooling region.
%
%Actually, the proposed $\cat$ activation scheme can be viewed as a maxout unit that performs cross-channel max pooling from the positive and negative phase of corresponding filters.

%Another way to view $\cat$ is that by treating the positive and negative phase equally, it heuristically conducts cross-channel pooling. 
%
%Spatial pooling has been well researched from many perspectives~\cite{zeiler2013stochastic,lee2015generalizing}. 
%
%But few endeavor to design effective cross-channel pooling because it is much more difficult to manually define the pooling region.
%
%~\citet{goodfellow2013maxout} studies the max-out network that learns which channel to activate while zeroing out the other channels. 
%
%For our proposed models, after $\cat$ separates the positive and negative activation and then applies non-linearity, the next conv layer directly functions as the cross-channel pooling operator.
%
%As a consequence of cross-channel pooling, models integrating $\cat$ are supposed to produce more invariant features. 
%
We measure the invariance scores using the evaluation metrics from~\citep{goodfellow2009measuring} and draw another comparison between the $\cat$ models and the $\relu$ models.
%
For a fair evaluation, we compare all 7 conv layers from all-conv $\relu$ model with those from all-conv $\cat$ model trained on CIFAR-10/100. 
%
In the case of ImageNet experiments, we choose the model where $\cat$ replaces $\relu$ for the first 7 conv layers and compare the invariance scores with the first 7 conv layers from the baseline $\relu$ model.
%
Section~\ref{invar_score} in the supplementary materials details how the invariance scores are measured. 
%
%For CIFAR-10/100, we utilize all 50k testing images to calculate the invariance scores; for ImageNet, we take the center crop images from 5k randomly sampled validation examples.
%%
%For each individual filter, we calculate its own \emph{firing} threshold, such that it is fired one percent of the time, i.e. the \emph{global firing rate} is $0.01$. 
%%
%To build the set of semantically similar stimuli for each testing image $x$, we apply horizontal flip, 15 degree rotation and translation.
%%
%For CIFARI-10/100, translation is composed of horizontal/vertical shifts by 3 pixels; for ImageNet, translation is composed of cropping from the 4 corners. 
%%
%Because our setup is convolutional, we consider a filter to be fired only if both the transformed stimulus and the original testing example activate the filter to a level above the threshold at the same spatial location.
%%
%At the end, for each conv layer, we average the invariance scores of all of its filters to form the final score. 

%
Figure~\ref{fig:invar_cifar} plots the invariance scores for networks trained on CIFAR-10, CIFAR-100, and ImageNet respectively. 
%
The invariance scores of $\cat$ models are consistently higher than those of $\relu$ models.
%With little ambiguity, the invariance scores of $\cat$ models for all convolution layers are higher than those of $\relu$ models.
%
For CIFAR-10 and CIFAR-100, there is a big increase between conv2 and conv3 then again between conv4 and conv6, which are due to max-pooling layer extracting shift invariance features. 
%
%We also observe that although as a general trend, the invariance scores increase while going deeper into the networks--consistent with the observations from~\citep{goodfellow2009measuring}, rather unexpectedly, the progression is not monotonic. 
We also observe that although as a general trend, the invariance scores increase while going deeper into the networks--consistent with the observations from~\citep{goodfellow2009measuring}, the progression is not monotonic. 
%Although as a general trend, the invariance scores increase while going deeper into the networks--consistent with the observations from~\citep{goodfellow2009measuring}, rather unexpectedly, the progression is not monotonic. 
%As a general trend, the invariance scores increase while going deeper into the networks---consistent with the observations from~\citep{goodfellow2009measuring}, but rather unexpectedly, the trend is not always monotonic. 
%
This interesting observation suggests the potentially diverse functionality of different layers in the CNN, which would be worthwhile for future investigation.

In particular, the scores of ImageNet $\relu$ model attain local maximum at conv1, conv4 and conv7 layers. It inspires us to design the architecture where $\cat$ are placed after conv1, 4, and 7 layers to encourage invariance representations while halving the number of filters to limit model capacity.
%
% Surprisingly yet as hoped, this architecture achieves the best top1 and top5 recognition results when averaging scores from $10$ patches.
Interestingly, this architecture achieves the best top1 and top5 recognition results when averaging scores from $10$ patches.
%
%This observation casts light on the diverse functionality in convolution layers, which would be worthwhile for future investigation.
%raises another interesting question that whether all conv layers are playing for future research : are all conv layers playing the same role?  
%%
%The simple answer is ``no''--in fact, for our VGG net experiments on CIFAR-10/100, replacing all conv1, conv2 and conv3 with $\cat$ produces worse results than both baseline+conv1 and baseline+(conv1,conv3) models. 
%%
%A natural follow-up question is: what are their individual roles then? 
%%
%There is no simple answer this time: some adds a little abstractness while preserving most information, some operates cross-channel pooling, some operates spatial pooling, some focus on generating non-linearity and etc.
%%
%Nonetheless, at the least, our experiments demonstrate that once we match $\cat$ with the right convolution layers, i.e. \ those who disentangle the phases and preserve most information, we can much better realize the potential of the networks. 


==> Discussions.tex <==
%\begin{figure*}[t]
%\centering
%\subfigure[conv1]{\includegraphics[width=0.22\textwidth]{figures/allconc3_conv1-crop.pdf}}\hspace{0.07in}
%\subfigure[conv2]{\includegraphics[width=0.22\textwidth]{figures/allconc3_conv2-crop.pdf}}\hspace{0.07in}
%\subfigure[conv3]{\includegraphics[width=0.22\textwidth]{figures/allconc3_conv3-crop.pdf}}\hspace{0.07in}
%\subfigure[conv4]{\includegraphics[width=0.22\textwidth]{figures/allconc3_conv4-crop.pdf}}
%\caption{\textbf{Histograms of $\mu^r$(dark blue) and $\mu^w$(yellow) for $\cat$ model on ImageNet.} The two distributions align with each other for all conv1-conv4 layers--as we expected, the pairing phenomenon is not present any more after applying $\cat$ activation scheme.
%}\label{fig:dist_allconc3}
%\end{figure*}



\begin{table}[t]
\caption{\textbf{Validation error rates on ImageNet.} We compare the performance of baseline model with the proposed $\cat$ models at different levels of activation scheme replacement. Error rates with $^\dagger$ are obtained by averaging scores from $10$ patches.\label{tab:AllConvResult}}
\vspace{0.05in}
\centering
\small
\begin{tabular}{c|c|c|c|c} 
\hline
Model & top-1 & top-5 & top-1$^\dagger$ & top-5$^\dagger$ \\ \hline
Baseline & 41.81 & 19.74  & 38.03  & 17.17 \\ \hline
$\abs$ (conv1--4) & 41.12 & 19.25 & 37.32   & 16.49 \\ \hline  
$\abs$ (conv1--7) &  42.36 & 20.05 & 38.21 & 17.42 \\ \hline
$\abs$ (conv1--9) & 43.33 & 21.05 & 39.70  & 18.39 \\ \hline
$\cat$ (conv1,4,7) & 40.45 &  18.58 & \textbf{35.70}   & \textbf{15.32} \\ \hline
$\cat$ (conv1--4) & \textbf{39.82} & \textbf{18.28} & 36.20   & 15.72 \\ \hline  
$\cat$ (conv1--7) &  39.97 & 18.33 & 36.53 & 16.01 \\ \hline
$\cat$ (conv1--9) & 40.15 & 18.58 & 36.50  & 16.14 \\ \hline
$\cat$ (all) & 40.93 & 19.39 & 37.28 & 16.72 \\ \hline
\end{tabular}
\vspace{-0.05in}
%The best model is AllConC1 where the first 4 conv layers are followed by $\cat$. Adding more $\cat$ does not keep improving the classification results. 
%It is also interesting to note that dropout does not necessarily help in this type of conv architecture.  
%\label{tab:AllConvResult}}
\end{table}


\begin{table}[t]
\caption{\textbf{Comparison to other methods on ImageNet.} We compare with AlexNet and other variants, such as  FastFood-32-AD (FriedNet)~\cite{yang2014deep} and pruned AlexNet (PrunedNet)~\cite{han2015learning}, which are modifications of AlexNet aiming at reducing the number of parameters, as well as All-CNN-B, the baseline model~\cite{springenberg2014striving}. Error rates with $^\dagger$ are obtained by averaging scores from $10$ patches.\label{tab:ImageNetResult}}
\vspace{0.05in}
\centering
\small
\begin{tabular}{c|c|c|c|c|c} 
\hline
Model & top-1 & top-5 & top-1$^\dagger$ & top-5$^\dagger$ & params. \\ \hline
AlexNet & 42.6 & 19.6   & 40.7 & 18.2 & $61$M \\ \hline
%VGGF & 41.4 &   19.1 & -- & -- &  60.8 \\ \hline
FriedNet & 41.93 & -- & -- & -- & $32.8$M \\ \hline
PrunedNet & 42.77 & 19.67 & -- & -- & $6.7$M \\ \hline
AllConvB & 41.81 & 19.74  & 38.03  & 17.17& $9.4$M \\ 
%ZeilerNet & -- & --   & 37.5 & 16.0 & $108$M \\
%AllConv& 41.81 & 19.74  & 38.03  & 17.17  & 9.3 \\ \hline
% AllConv dropout& 42.06 &  19.86 & 38.50 & 17.32 & 9.3 \\ \hline
\thickhline
$\cat$ (all) & 40.93 & 19.39 & 37.28 & 16.72 & $\mathbf{4.7}$M \\ \hline
(conv1,4,7) & 40.45 &  18.58 & \textbf{35.70}   & \textbf{15.32} & 8.6 M \\ \hline
%AllConC1& 40.39  & 18.64 & 36.47  & 16.16  & 16.6 \\ \hline
%AllConC1 dropout& 40.15 & 18.58 & 36.50  & 16.14  & 16.6 \\ \hline
%AllConC2& 40.67 & 18.52 & 36.63  & 15.92  & 11.6  \\ \hline
%AllConC2 dropout&  39.97 & 18.33 & 36.53 & 16.01 & 11.6 \\ \hline
(conv1--4) & \textbf{39.82} & \textbf{18.28} & 36.20   & 15.72 & $10.1$M  \\ \hline
%AllConC3 dropout& 40.55   & 18.61 & 16.22 & 36.87  & 10 \\ \hline
\end{tabular}
\vspace{-0.05in}
%
%By comparison, our AllConCh model shrinks the size of the network the most yet improves in classification performance and our AllConC1 achieves the best results with comparable number of parameters as PrunNet. 
%
%We also include results from Zeiler Net~\cite{zeiler2014visualizing}, which has the same number of conv layers as AlexNet but sufficiently different architecture.
%
%.}\label{tab:ImageNetResult}
\end{table}

\cutsectionup
\section{Discussion}
\label{sec:discussion}
%The experiments on CIFAR and ImageNet datasets in turn provide us with more insight into the behavior of $\cat$. %, which is discussed in this section.
%
In this section, we discuss qualitative properties of $\cat$ activation scheme in several viewpoints, such as regularization of the network and learning invariant representation.
%as well as disentangling and reconstruction properties of the network.
%
\begin{figure*}[htbp]
\centering
\subfigure[CIFAR-10]{\label{fig:cifar100_traintest}\includegraphics[height=1.5in]{figures/invar_cifar10.png}}
\subfigure[CIFAR-100]{\label{fig:cifar100_test}\includegraphics[height=1.5in]{figures/invar_cifar100.png}}
\subfigure[ImageNet]{\label{fig:cifar100_test}\includegraphics[height=1.5in]{figures/invar_imagenet.png}}
\vspace{-0.1in}
\caption{\textbf{Invariance Scores for $\relu$ Models vs $\cat$ Models}. The invariance scores for $\cat$ models are consistently higher than $\relu$ models. The invariance scores jump after max-pooling layers. Moreover, even though the invariance scores tend to increase along with the depth of the networks, the progression is not monotonic.\label{fig:invar_cifar}}
\vspace{-0.1in}
\end{figure*}

\input{Regularization}
\input{CrossChannel}
\input{FeatureLearning}


==> Experiments.tex <==

\begin{table*}[t]
\caption{\textbf{Test set recognition error rates on CIFAR-10/100.} We compare the performance of $\relu$ models (baseline) and $\cat$ models with different model capacities: ``double" refers to the models that double the number of filters and ``half" refers to the models that halve the number of filters. The error rates are provided in multiple ways, such as ``Single", ``Average" (with standard error), or ``Vote", based on cross-validation methods. We also report the corresponding train error rates for the Single model. The number of model parameters are given in million. Please see the main text for more details about model evaluation.\label{tab:cifar_results}}
\vspace{0.05in}
\centering
\small
\begin{tabular}{c|c|c|c|c|c|c|c|c|c} 
\hline
\multirow{3}{*}{Model} & \multicolumn{4}{c|}{CIFAR-10} & \multicolumn{4}{c|}{CIFAR-100} & \multirow{3}{*}{params.}\\ \cline{2-9}
 & \multicolumn{2}{c|}{Single} & \multirow{2}{*}{Average} & \multirow{2}{*}{Vote} & \multicolumn{2}{c|}{Single} & \multirow{2}{*}{Average} & \multirow{2}{*}{Vote} &  \\ \cline{2-3}\cline{6-7}
 & train & test &  &  & train & test &  &  &  \\ \hline
Baseline & 1.09 & 9.17 & 10.20{\scriptsize$\pm 0.09$} & 7.55 & 13.68 & 36.30 & 38.52{\scriptsize$\pm 0.12$} & 31.26 & $1.4$M \\
{\small$+$} (double) & 0.47 & 8.65 & 9.87{\scriptsize$\pm 0.09$} & 7.28 & 6.03 & 34.77 & 36.73{\scriptsize$\pm 0.15$} & 28.34 & $5.6$M \\ \hline
$\abs$ & 4.10 & {\bf 8.32} & 10.26{\scriptsize$\pm 0.10$} & 7.76 & 19.35 & 35.00 & 37.24{\scriptsize$\pm 0.20$} & 29.77 & $1.4$M \\ \hline
$\cat$ & 4.23 & 8.43 & \bf{9.39}{\scriptsize$\pm 0.11$} & \bf{7.09} & 14.25 & {\bf 31.48} & \bf{33.76}{\scriptsize$\pm 0.12$} & {\bf 27.60} & $2.8$M \\ 
{\small$+$} (half) & 4.73 & {\bf 8.37} & \bf{9.44}{\scriptsize$\pm 0.09$} & {\bf 7.09} & 21.01 & 33.68 & 36.20{\scriptsize$\pm 0.18$} & 29.93 & $0.7$M \\ 
%\multicolumn{5}{c}{CIFAR-100}\\ \hline
%Model & Single & Average & Vote & params. \\ \hline
%Baseline & 36.30 (13.68) &    38.52{\scriptsize$\pm 0.12$} & 31.26 & $1.4$M \\
%{\small$+$} (double) & 34.77 (6.03) &    36.73{\scriptsize$\pm 0.15$} & 28.34 & $5.6$M \\ \hline
%$\cat$ & \bf{31.48} (14.25)&    \bf{33.76}{\scriptsize$\pm 0.12$} & \bf{27.60} & $2.8$M \\
%{\small$+$} (half) & 33.68 (21.01) &    36.20{\scriptsize$\pm 0.18$} & 29.93 & $0.7$M \\ \hline
%\hline
\hline
\end{tabular}
\vspace{-0.1in}
\end{table*}


\cutsectionup
\section{Benchmark Results}
\label{sec:experiments}
%We  evaluate  $\cat$  on  three  benchmark datasets and boost the baseline performances on all of them, with little additional hyperparameter tuning .
%%
%We strive for simple architecture and simple optimization techniques in order to directly assess the impact of $\cat$. 
%%
%Therefore, the CNN models introduced by~\citep{springenberg2014striving} serve our purpose well, where convolution, $\relu$, average-pooling and max-pooling (for CIFAR10/100 only) are the sole building blocks of these networks.
%%
%The only regularization techniques we apply during training are dropout~\cite{srivastava2014dropout} and weight decay if optimizing with SGD.
%
We evaluate the effectiveness of the $\cat$ activation scheme on three benchmark datasets: CIFAR-10, CIFAR-100~\cite{krizhevsky2009learning} and ImageNet~\cite{deng2009imagenet}.
%
To directly assess the impact of $\cat$, we employ existing CNN architectures with $\relu$ that have already shown a good recognition baseline and demonstrate improved performance on top by replacing $\relu$ into $\cat$.
%
%
Note that the models with $\cat$ activation don't need significant hyperparameter tuning from the baseline $\relu$ model, and in most of our experiments, we only tune dropout rate while other hyperparameters (e.g., learning rate, mini-batch size) remain the same.
%
We also replace $\relu$ with $\abs$ for comparison with $\cat$.
%Due to page limit, 
The details of network architecture are in Section~\ref{sec:model} of the supplementary materials.
%\begin{figure*}[t]
%\centering
%%\subfigure[CIFAR-10\label{fig:cifar10_progression}]{\includegraphics[height=1.7in]{figures/cifar10-plot.pdf}}\hspace{0.1in}
%%\subfigure[CIFAR-100\label{fig:cifar100_progression}]{\includegraphics[height=1.7in]{figures/cifar100-plot.pdf}}
%\subfigure[CIFAR-10\label{fig:cifar10_progression}]{\includegraphics[height=1.5in, width = 2.8in]{figures/cifar-10_smooth_4.pdf}}\hspace{0.3in}
%\subfigure[CIFAR-100\label{fig:cifar100_progression}]{\includegraphics[height=1.5in, width = 2.8in]{figures/cifar-100_smooth_4.pdf}}
%\vspace{-0.1in}
%\caption{\textbf{Progression of train and test set error rates on CIFAR-10/100.}\label{fig:cifar_progression}}
%\vspace{-0.1in}
%\end{figure*}

\cutsubsectionup
\subsection{CIFAR-10 and CIFAR-100}
\label{sec:exp-cifar}
%
The CIFAR-10 and 100 datasets~\cite{krizhevsky2009learning} each consist of $50,000$ training and $10,000$ testing examples of $32\times 32$ images evenly drawn from 10 and 100 classes, respectively.
%  
We subtract the mean and divide by the standard deviation for preprocessing and use random horizontal flip for data augmentation.
%
%\paragraph{Network Architecture.} Section~\ref{sec:cifarmodel} describes each model mentioned below in table format.
 
%
We use the ConvPool-CNN-C model~\citep{springenberg2014striving} as our baseline model, which is composed of convolution and pooling followed by $\relu$ without fully-connected layers.
%
This baseline model serves our purpose well since it has clearly outlined network architecture only with convolution, pooling, and $\relu$. 
%
It has also shown competitive recognition performance using a fairly small number of model parameters. 
%The baseline model for CIFAR-10/100 is the Conv-Pool CNN C, we refer to as \textbf{ConPo} (see Table~\ref{conpo}) from~\citep{springenberg2014striving}.
%
%We choose this model because (1) it has a clearly outlined topology--$3\times 3$ convolution of stride $1$ followed by $3\times 3$ max-pooling of stride $2$, (2) it achieves state-of-the-art level performances based on the results reported by \citep{springenberg2014striving} and (3) its high parameter-efficiency ($1.4$ million parameters) enables us to conduct sufficient control experiments to rigorously assess $\cat$. 
%

First, we integrate $\cat$ into the baseline model by simply replacing $\relu$ while keeping the number of convolution filters the same.
%
This doubles the number of output channels at each convolution layer and the total number of model parameters is doubled.
%
To see whether the performance gain comes from the increased model capacity, we conduct additional experiments with the baseline model while doubling the number of filters and the $\cat$ model while halving the number of filters.
%
We also evaluate the performance of the $\abs$ model while keeping the number of convolution filters the same as the baseline model.

%
Since the datasets don't provide pre-defined validation set, we conduct two different cross-validation schemes:
%
\begin{enumerate}[itemsep=5pt,nolistsep]
\item{``Single": we hold out a subset of training set for initial training and retrain the network from scratch using the whole training set until we reach at the same loss on a hold out set~\cite{goodfellow2013maxout}. For this case, we also report the corresponding train error rates.}
\item{$10$-folds: we divide training set into $10$ folds and do validation on each of $10$ folds while training the networks on the rest of $9$ folds. The mean error rate of single network (``Average") and the error rate with model averaging of $10$ networks (``Vote") are reported.}
%
\end{enumerate}
%
%\begin{table}[t]
%\centering
%\small
%\begin{tabular}{c|c|c|c|c} 
%\hline
%\multicolumn{5}{c}{CIFAR-10}\\ \hline
%Model & Single (train) & Average & Vote & params. \\ \hline
%Baseline & 9.17 (1.09) &    10.20{\scriptsize$\pm 0.09$} & 7.55 & $1.4$M \\
%{\small$+$} (double) & 8.65 (0.47) &    9.87{\scriptsize$\pm 0.09$} & 7.28 & $5.6$M \\ \hline
%$\cat$ & \bf{8.43} (4.23) &    \bf{9.39}{\scriptsize$\pm 0.11$} & \bf{7.09} & $2.8$M \\ 
%{\small$+$} (half) & \bf{8.37} (4.73) &    \bf{9.44}{\scriptsize$\pm 0.09$} & \bf{7.09} & $0.7$M \\ \hline\hline
%\multicolumn{5}{c}{CIFAR-100}\\ \hline
%Model & Single & Average & Vote & params. \\ \hline
%Baseline & 36.30 (13.68) &    38.52{\scriptsize$\pm 0.12$} & 31.26 & $1.4$M \\
%{\small$+$} (double) & 34.77 (6.03) &    36.73{\scriptsize$\pm 0.15$} & 28.34 & $5.6$M \\ \hline
%$\cat$ & \bf{31.48} (14.25)&    \bf{33.76}{\scriptsize$\pm 0.12$} & \bf{27.60} & $2.8$M \\
%{\small$+$} (half) & 33.68 (21.01) &    36.20{\scriptsize$\pm 0.18$} & 29.93 & $0.7$M \\ \hline
%\hline
%\end{tabular}
%\vspace{-0.05in}
%\caption{\textbf{Test set recognition error on CIFAR-10/100.} We compare the performance of $\relu$ models (baseline) and $\cat$ models with different model capacity: ``double" refers the model that doubles the number of filters and ``half" refers the model that halves the number of filters. The error rates are provided in multiple ways, such as ``Single", ``Average" (with standard error), or ``Vote", based on cross-validation methods. We also report the corresponding train error rate in $(\cdot)$ for the Single case. The $\#$ of model parameters are given in million. \label{tab:cifar_results}}
%\vspace{-0.1in}
%\end{table}

%
%\begin{center}
%\begin{table}[t]
%    \begin{tabular}{  p{1.5cm} |  l  |  l  |  l |  l } 
%    \hline
%    Model & Single & CV Average & CV Mix & PM \\ \hline
%    ConPo & 36.3 &    38.5 $\pm$ 0.37  & 31.3 & 1.4 \\ \hline
%    CoPoD & 34.8 &    36.3 $\pm$ 0.48  & 28.3 & 5.6 \\ \hline
%    CoPoCh & 33.7 &    36.2 $\pm$ 0.57  & 29.9 & \textbf{0.7} \\ \hline
%    CoPoC & \textbf{31.5} & \textbf{33.8 $\pm$ 0.39}  & \textbf{27.6} & 2.8 \\ \hline
%    \hline
%    \end{tabular}
%   \caption{\textbf{CIFAR-100 Testing Results}. Similarly with Table~\ref{Cifar10Result}, we compare $\relu$ with $\cat$. The impact of $\cat$ in enhancing the network performance is more evident for CIFAR-100. }\label{Cifar100Result}
%\end{table}
%\end{center}
%
The recognition results are summarized in Table~\ref{tab:cifar_results}.
%
On CIFAR-10, we observe significant improvement with the $\cat$ activation over $\relu$.
%
Especially, $\cat$ models consistently improve over $\relu$ models with the same number of neurons (or activations) while reducing the number of model parameters by half (e.g., $\cat$ + half model and the baseline model have the same number of neurons while the number of model parameters are $0.7$M and $1.4$M, respectively).
%
On CIFAR-100, the models with larger capacity generally improve the performance for both activation schemes. 
%
Nevertheless, we still find a clear benefit of using $\cat$ activation that shows significant performance gain when it is compared to the model with the same number of neurons, i.e., half the number of model parameters.
%
One possible explanation for the benefit of using $\cat$ is its regularization effect, as can be confirmed in Table~\ref{tab:cifar_results} that the $\cat$ models showed significantly lower gap between train and test set error rates than those of the baseline $\relu$ models.
%

To our slight surprise, $\abs$ outperforms the baseline $\relu$ model on CIFAR-100 with respect to all evaluation metrics and on CIFAR-10 with respect to single-model evaluation. 
%
%It also reaches promising single-model recognition accuracy comparing to $\cat$ on CIFAR-10--but likely owing to a lucky initialization: 
It also reaches promising single-model recognition accuracy compared to $\cat$ on CIFAR-10; however, when averaging or voting across 10-folds validation models, $\abs$ becomes clearly inferior to $\cat$.  
%
%It appears that the quality of each $\abs$ model varies substantially, which can be an additional disadvantage in practice.
%\paragraph{Result Summary.} 
%%
%The  for CIFAR-10 are summarized in Table~\ref{Cifar10Result} and CIFAR-100 in Table~\ref{Cifar100Result}; the training-vs-testing error rate curves over epochs are presented in Figure~\ref{fig:cifar_test}.
%%
%CIFAR-10, with only 10 classes and more training examples from each class, presents an easier classification task than CIFAR-100. 
%%
%Intuitively, the model capacity to achieve the best result for CIFAR-100 ought to be higher than that for CIFAR-10. 
%%
%Indeed, the most competitive model for CIFAR-10 is CoPoCh: it performs at the same level as CoPoC but with the least number of parameters.
%%
%For CIFAR-100, with a higher capacity, CoPoC outperforms CoPoCh and similarly CoPoD outperforms ConPo; CoPoCh still outperforms both ConPo and CoPoD when evaluating on individual models, whereas CoPoC consistently improves this line of networks by a significant margin.
%%
%Since the classification performance for CIFAR-100 is not as saturated as CIFAR-10, we can better witness the effect of $\cat$ in improving the CNN models from CIFAR-100 experiments. 
%%
%Such effect, furthermore, cannot be simply replaced by adding more hidden units.
%%
%We present more analysis on CIFAR experiments Section~\ref{sec:discussions}. 
%%\paragraph{CIFAR-10}  



%To integrate $\cat$ into our baseline architecture, Our \textbf{CoPoC} (see Table~\ref{copoc}) model add $\cat$ after each conv layer in ConPo and keep the same number of filters. 
%
%The total number of parameters is thus doubled ($2.8$ million).
%

%Similarly, we build our \textbf{CoPoCh} (see Table~\ref{copoch}) model but reduce the number of filters at each conv layer by half\footnote{For CoPoCh, we apply $\cat$ to the input as well, hence the first layer conv filters are of dimension $6\times 48$.}.
%
%The total number of parameters is thus halfened ($1.4$ million).

%Lastly, to demonstrate that the boost in classification through \textbf{CoPoC} is not purely due to the increased model capacity, we train another model, \textbf{CoPoD} (see Table~\ref{copod}), by doubling the filters in each conv layer from ConPo but without using $\cat$. 
%
%The total number parameters is thus quadrupled ($5.6$ million).

%\paragraph{Training Details.} All of the above networks are optimized using Adam~\cite{kingma2014adam} with an initial learning rate $0.0002$ and mini-batch size of $100$ examples for $800$ epochs.   
%
%The dropout ratio for ConPo, CoPoC, CoPoD after each conv layer is $0.3$, for CoPoCh is $0.2$.

%\paragraph{Evaluation Metric.} 
%%
%Due to the lack of a pre-defined validation set, there has not been a universal method in evaluating CIFAR-10/100. 
%%
%To make the most fair comparison, we split the training images into 10 fold for cross validation.
%%
%We select the model\footnote{In reality, due to lack of space, our check-point is set to every 25 epochs.} that performs the best for each fold on the corresponding validation data, report the averaged results from applying individual models on the testing set and also report the results from the mixture of all models. 
%%
%Finally, based on our cross validation results, we train all models from scratch using all the training data and report results from a single model on the testing set, following the single-model evaluation metric from~\cite{goodfellow2013maxout}.



%\paragraph{Result Summary.} 
%%
%The results for CIFAR-10 are summarized in Table~\ref{Cifar10Result} and CIFAR-100 in Table~\ref{Cifar100Result}; the training-vs-testing error rate curves over epochs are presented in Figure~\ref{fig:cifar_test}.
%%
%CIFAR-10, with only 10 classes and more training examples from each class, presents an easier classification task than CIFAR-100. 
%%
%Intuitively, the model capacity to achieve the best result for CIFAR-100 ought to be higher than that for CIFAR-10. 
%%
%Indeed, the most competitive model for CIFAR-10 is CoPoCh: it performs at the same level as CoPoC but with the least number of parameters.
%%
%For CIFAR-100, with a higher capacity, CoPoC outperforms CoPoCh and similarly CoPoD outperforms ConPo; CoPoCh still outperforms both ConPo and CoPoD when evaluating on individual models, whereas CoPoC consistently improves this line of networks by a significant margin.
%%
%Since the classification performance for CIFAR-100 is not as saturated as CIFAR-10, we can better witness the effect of $\cat$ in improving the CNN models from CIFAR-100 experiments. 
%%
%Such effect, furthermore, cannot be simply replaced by adding more hidden units.
%%
%We present more analysis on CIFAR experiments Section~\ref{sec:discussions}. 
%%\paragraph{CIFAR-10}  
%\begin{figure*}[t]
%     %\begin{center}
%%
%        \subfigure[CIFAR-10]{%
%            \label{fig:cifar10_traintest}
%            \includegraphics[width=8cm, height=5cm]{figures/cifar10_traintest.png}
%        }%
%          \hspace{2em}
%        \subfigure[CIFAR-100]{%
%           \label{fig:cifar100_traintest}
%           \includegraphics[width=8cm, height=5cm]{figures/cifar100_traintest.png}
%        }%  ------- End of the first row ----------------------%
%   % \end{center}
%\caption{\textbf{CIFAR-10/100 Results}. We plot the training and test error rate (in $\%$) for CIFAR-10 and CIFAR-100. We can see that $\cat$ models outperforms $\relu$ models--the trend is more obvious for CIFAR-100. \label{fig:cifar_test}}
% \end{figure*}
%
%\begin{center}
%\begin{table}[t]
%    \begin{tabular}{   p{1.5cm} |  l  |  l  |  l |  l } 
%    \hline
%    Model & Single & CV Average & CV Mix & PM \\ \hline
%    ConPo & 9.2 &    10.2 $\pm$ 0.29  & 7.6 & 1.4 \\ \hline
%    CoPoD & 8.6 &    9.9 $\pm$ 0.28  & 7.3 & 5.6 \\ \hline
%    CoPoCh & \textbf{8.4} &    \textbf{9.4 $\pm$ 0.27}  & \textbf{7.1} & \textbf{0.7} \\ \hline
%    CoPoC & 8.4 &    9.4 $\pm$ 0.35  & 7.1 & 2.8 \\ \hline
%    \hline
%    \end{tabular}
%   \caption{\textbf{CIFAR-10 Testing Results}. We compare the two models with generic $\relu$ activation with our proposed models with $\cat$. We show error rates in $\%$ evaluated in 3 differen ways. \emph{Single} shows the result of a single model's testing performance, trained on the entire training dataset and selected by the evaluation metric in~\citep{goodfellow2013maxout}. \emph{CV Average} is the mean of the indiviudal performances on the testing data from the 10 models obtained during cross validation. \emph{CV Mix} is the result on the testing data by mixing the softmax layer outputs from the 10 models. PM is the number of parameters (in million). }\label{Cifar10Result}
%\end{table}
%\end{center}

%\paragraph{CIFAR-100}
%\begin{figure*}[t]
    % \begin{center}
%
%        \subfigure[Accuracy for training and test dataset over epochs.]{%
%            \label{fig:cifar100_traintest}
  %          \includegraphics[width=8cm, height=5cm]{figures/cifar100_traintest.png}
%        }%
 %         \hspace{2em}
  %      \subfigure[Zoomed-in test accuracy.]{%
   %        \label{fig:cifar100_test}
    %       \includegraphics[width=8cm, height=5cm]{figures/cifar100_test.png}
 %       }%  ------- End of the first row ----------------------%
   % \end{center}
%\caption{\textbf{CIFAR-100 Results}. We plot the training and test error rate (in $\%$) for CIFAR-100 in Figure~\ref{fig:cifar100_traintest}, when trained on the entire training set. We also zoom in to the last 400 epochs to have a closer look (Figure~\ref{fig:cifar100_test}); both $\cat$ models significantly outperform both $\relu$ models. \label{fig:cifar10_test}}
 %\end{figure*}
%
%\begin{center}
%\begin{table}[t]
%    \begin{tabular}{  p{1.5cm} |  l  |  l  |  l |  l } 
%    \hline
%    Model & Single & CV Average & CV Mix & PM \\ \hline
%    ConPo & 36.3 &    38.5 $\pm$ 0.37  & 31.3 & 1.4 \\ \hline
%    CoPoD & 34.8 &    36.3 $\pm$ 0.48  & 28.3 & 5.6 \\ \hline
%    CoPoCh & 33.7 &    36.2 $\pm$ 0.57  & 29.9 & \textbf{0.7} \\ \hline
%    CoPoC & \textbf{31.5} & \textbf{33.8 $\pm$ 0.39}  & \textbf{27.6} & 2.8 \\ \hline
%    \hline
%    \end{tabular}
%   \caption{\textbf{CIFAR-100 Testing Results}. Similarly with Table~\ref{Cifar10Result}, we compare $\relu$ with $\cat$. The impact of $\cat$ in enhancing the network performance is more evident for CIFAR-100. }\label{Cifar100Result}
%\end{table}
%\end{center}
%
\paragraph{Experiments on Deeper Networks.} 
%
We conduct experiments with very deep CNN that has a similar network architecture to the VGG network~\cite{simonyan2014very}.
%
Specifically, we follow the model architecture and training procedure in~\citet{Zblog}.
%
%The model architecture and training procedure are described in details by~\citet{Zblog} in the related blog post. 
%For data augmentation, we use random shifts in addition to random horizontal flip.
%
%Since this paper does not intend to carry out state-of-the-art results, we follow the training procedure reported in the post exactly with no further tuning for 400 epochs.
%
Besides the convolution and pooling layers, this network contains batch normalization~\cite{ioffe2015batch} and fully connected layers. %, which are important building blocks when training on the relatively small CIFAR datasets.
%
Due to the sophistication of the network composition which may introduce complicated interaction with $\cat$, we only integrate $\cat$ into the first few layers.
%
%
Similarly, we subtract the mean and divide by the standard deviation for preprocessing and use horizontal flip and random shifts for data augmentation. %for data augmentation, we use random horizontal flip as well as random shifts. 


%
In this experiment\footnote{We attempted to replace $\relu$ with $\abs$ on various layers but we observed significant performance drop with $\abs$ non-linearity when used for deeper networks.}, we gradually replace $\relu$ after the first, third, and the fifth convolution layers\footnote{Integrating $\cat$ into the second or fourth layer before max-pooling layers did not improve the performance.} with $\cat$ while halving the number of filters, resulting in a reduced number of model parameters. % as we replace more $\relu$ into $\cat$ activations.
%
%See Table~\ref{vgg}, \ref{vgg1}, \ref{vgg3}, and \ref{vgg5} in the supplementary material for details of architecture.
%
We report the test set error rates using the same cross-validation schemes as in the previous experiments. 
%
As shown in Table~\ref{tab:VGGresult}, there is substantial performance gain in both datasets by replacing $\relu$ with $\cat$.
%
Overall, the proposed $\cat$ activation improves the performance of the state-of-the-art VGG network significantly, achieving highly competitive error rates to other state-of-the-art methods, as summarized in Table~\ref{tab:cifar_compare}.
%
%The number of filters for each layer with $\cat$ are halved

%We also swap the $\relu$ of first few layers with $\abs$. 
%%
%Unfortunately, the performance of the single-model error rates for all our attempts are at the least $5\%$ behind the baseline VGG model. 
%%
%These results indicate $\abs$'s incompatibility with deep network architecture and  we do not proceed with more extensive experiments. 
%
%\textbf{VGG1} replaces $\relu$ after conv1 with $\cat$;  \textbf{VGG3} replaces $\relu$ after conv1, conv3 with $\cat$; \textbf{VGG5} replaces $\relu$ after conv1, conv3, conv5 with $\cat$.
%
%We also reduce the number of filters to half if $\cat$ is applied instead of $\relu$ (see Table~\ref{vgg},~\ref{vgg1},~\ref{vgg3} and~\ref{vgg5}).
%
%In other words, the more $\relu$ being replaced by $\cat$, the fewer the parameters there are. 
%
%For each model, we report the result of the last epoch in Table~\ref{VGGResult}. 
%
%We graph the training and testing curves for a more visual comparison in Figure~\ref{fig:cifar_vgg}. 
%
%From our experiments, we can more affirmatively conclude that $\cat$ can enhance the performances of very deep CNNs, when applied on the first few conv layers. 
%
%There have been a variety of works focusing on carrying out state-of-the-art CIFAR-10/100 results. 
%%
%The degree of network architecture, size of the model, hyperparameter tuning, regularization techniques, training procedure, data augmentation, data pre-processing and evaluation metric covers too wide a spectrum to make a scientifically fair comparison. 
%%
%Nonetheless, we collect some published results in Table~\ref{cifar_compare} for readers' references. 

%\begin{table}[t]
%\centering
%\small
%\begin{tabular}{c|c|c|c|c} 
%\hline
% & VGG & (conv1) & (conv1,3) & (conv1,3,5) \\ \hline
%CIFAR-10 & 6.55 & 6.37 & \bf{6.01} & 6.14  \\ \hline
%CIFAR-100 & 29.28& 27.25& 26.70& \bf{26.22}  \\ \hline 
%\hline
%\end{tabular}
%\vspace{-0.05in}
%\caption{\textbf{Test set recognition error on CIFAR-10/100 using deeper networks.} We gradually apply $\cat$ in replace of $\relu$ for conv1, 3, and conv5 layers of baseline VGG network while halving the number of convolution filters.\label{tab:VGGresult}}
%\vspace{-0.05in}
%\end{table}

\begin{table}[t]
%\caption{\textbf{Test set recognition error rates on CIFAR-10/100 using deeper networks.} We gradually apply $\cat$ in replace of $\relu$ after conv1, conv3, and conv5 layers of the baseline VGG network while halving the number of convolution filters.\label{tab:VGGresult}}
\caption{\textbf{Test set recognition error rates on CIFAR-10/100 using deeper networks.} We gradually apply $\cat$ to replace $\relu$ after conv1, conv3, and conv5 layers of the baseline VGG network while halving the number of convolution filters.\label{tab:VGGresult}}
\vspace{0.05in}
\centering
\small
\begin{tabular}{c|c|c|c} 
\hline
\multicolumn{4}{c}{CIFAR-10}\\ \hline
Model & Single & Average & Vote  \\ \hline
VGG & 6.35 &    6.90{\scriptsize$\pm 0.03$} & 5.43  \\ \hline
(conv1) & 6.18  &    \bf{6.45}{\scriptsize$\pm 0.05$} & 5.22  \\ \hline
(conv1,3) &  \bf{5.94} &    \bf{6.45}{\scriptsize$\pm 0.02$} & \bf{5.09} \\  \hline
(conv1,3,5) & 6.06 &    \bf{6.45}{\scriptsize$\pm 0.07$} & 5.16 \\ \hline\hline
\multicolumn{4}{c}{CIFAR-100}\\ \hline
Model & Single & Average & Vote \\ \hline
VGG & 28.99 &   30.27{\scriptsize$\pm 0.09$} & 26.85  \\ \hline
(conv1) & 27.29 &   28.43{\scriptsize$\pm 0.11$} & 24.67 \\ \hline
(conv1,3) & 26.52 &  27.79{\scriptsize$\pm 0.08$} & 23.93  \\ \hline
(conv1,3,5) & \bf{26.16}  &  \bf{27.67}{\scriptsize$\pm 0.07$} & \bf{23.66}  \\ \hline
\end{tabular}
\vspace{-0.1in}
%We compare the two models with generic $\relu$ activation with our proposed models with $\cat$. We show error rates in $\%$ evaluated in 3 differen ways. \emph{Single} shows the result of a single model's testing performance, trained on the entire training dataset and selected by the evaluation metric in~\citep{goodfellow2013maxout}. \emph{CV Average} is the mean of the indiviudal performances on the testing data from the 10 models obtained during cross validation. \emph{CV Mix} is the result on the testing data by mixing the softmax layer outputs from the 10 models. PM is the number of parameters (in million). }\label{Cifar10Result}
\end{table}




\cutsubsectionup
\subsection{ImageNet}
\label{sec:exp-imagenet}
%
To assess the impact of $\cat$ on large scale dataset, we perform experiments on ImageNet dataset~\cite{deng2009imagenet}\footnote{We used a version of ImageNet dataset for ILSVRC 2012.}, which contains about $1.3$M images for training and $50,000$ for validation from $1,000$ object categories.
%
%For preprocessing, we subtract the estimated (with 1000 randomly selected training images) channel-wise mean and divide by the estimated channel-wise standard deviation.
For preprocessing, we subtract the mean and divide by the standard deviation for each input channel, and follow the data augmentation as described in~\cite{krizhevsky2012imagenet}.
%estimated (with 1000 randomly selected training images) channel-wise mean and divide by the estimated channel-wise standard deviation.
%
%For data augmentation, we follow the same procedure as in~\citet{krizhevsky2012imagenet}. 
%
%\vspace{-0.5em}
%\paragraph{Network Architecture\footnote{Section~\ref{sec:imagenetmodel} describes each model in detailed table format.}}

%
We take the All-CNN-B model~\citep{springenberg2014striving} as our baseline model. %\footnote{See Table~\ref{allconv} in the supplementary material for detailed network architecture.} as our baseline model. 
%
The network architecture of All-CNN-B is similar to that of AlexNet~\cite{krizhevsky2012imagenet}, where the max-pooling layer is replaced by convolution with the same kernel size and stride, the fully connected layer is replaced by $1\times1$ convolution layers followed by average pooling, and the local response normalization layers are discarded.
%
In sum, the layers other than convolution layers are replaced or discarded and finally the network consists of convolution layers only. 
%In sum, the layers other than convolution layers are replaced or discarded and finally the network consists of convolution layers only. 
%
We choose this model since it reduces the potential complication introduced by $\cat$ interacting with other types of layers, such as batch normalization or fully connected layers.
%
%The reason for us to choose AllConv as our baseline model is two-fold: the network consists of convolution layers only--such clean-cut architecture reduces the potential complication introduced by $\cat$ interacting with other types of layers, such as batch-normalization, max-pooling and fully-connected; AllConv has the least number of parameters comparing with other networks that have similar performances on ImageNet, which allows us to conduct more experiments using limited computation resources in a short amount of time. 
%

\begin{table}[t]
\caption{\textbf{Comparison to other methods on CIFAR-10/100.}\label{tab:cifar_compare}} %We compare the performance of VGG network with $\cat$ to other methods.% The training details of recently published works on CIFAR datasets cover too wide a spectrum to make a scientific comparison. This table is primarily for reader's reference. 
\vspace{0.05in}
\centering
\small
\begin{tabular}{c|c|c}
\hline
Model & CIFAR-10 & CIFAR-100  \\ \hline
\citep{rippel2015spectral} & 8.60 &  31.60   \\ \hline
\citep{snoek2015scalable} & 6.37 & 27.40   \\ \hline 
\citep{liang2015recurrent} & 7.09 & 31.75   \\ \hline 
\citep{lee2015generalizing} & 6.05  & 32.37  \\ \hline 
\citep{srivastava2015training} & 7.60 & 32.24   \\ \thickhline
VGG & 5.43 & 26.85 \\ \hline
VGG + $\cat$ & \textbf{5.09}  & \textbf{23.66}   \\ \hline 
\end{tabular}
\vspace{-0.05in}
\end{table} 


%
We gradually integrate more convolution layers with $\cat$ (e.g., conv1--4, conv1--7, conv1--9), while keeping the same number of filters. 
%
These models contain more parameters than the baseline model.
%and are trained using SGD..
%, in this experiments, keeping the same number of filters.
%
% We also evaluate two models where one replaces all $\relu$ layers into $\cat$ and the other conv1,conv4 and conv7 only, and both reduce the number of convolution layers before $\cat$ by half.
We also evaluate two models where one replaces all $\relu$ layers into $\cat$ and the other conv1,conv4 and conv7 only, where both models reduce the number of convolution layers before $\cat$ by half.
%
Hence, these models contain fewer parameters than the baseline model.
%
For comparison, $\abs$ models are also constructed by gradually replacing $\relu$ in the same manner as the $\cat$ experiments (conv1--4, conv1--7, conv1--9). 
%
%and work the best when trained with Adam~\cite{kingma2014adam}, an advanced stochastic optimization algorithm with adaptive learning rate schedule.
%All these networks except for  the last two are trained using SGD with mini-batch size of $64$ and momentum $0.9$; the last two models, both containing fewer parameters than the baseline model, %replaces all $\relu$ into $\cat$, 
%work the best when trained with Adam~\cite{kingma2014adam}, an advanced stochastic optimization algorithm with adaptive learning rate schedule.
%
The network architectures and the training details are in Section~\ref{sec:model} and Section~\ref{sec:detail-training} of the supplementary materials. %are in the supplementary material in Table~\ref{allconc1}, \ref{allconc2}, \ref{allconc3}, and \ref{allconch}.
%

%: \textbf{AllConC1} (Table~\ref{allconc1}) replacing the $\relu$ activation after conv1-conv4 layers with $\cat$; \textbf{AllConC2} (Table~\ref{allconc2}) conv1-conv7; \textbf{AllConC3} conv1-conv9 (Table~\ref{allconc3}).  

%Additionally, we build \textbf{AllConCh} model (Table~\ref{allconch}) where all the $\relu$ layers are replaced with $\cat$ and  the number of filters at each conv layer is reduced by half. 
%

%\paragraph{Training Details.} All of the above networks except for AllConCh are optimized using SGD with mini-batch size of $64$ examples and fixed momentum $0.9$. The learning rate and weight decay is adapted using the following schedule: epoch 1-10, $1\mathrm{e}{-2}$ and $5\mathrm{e}{-4}$; epoch 11-20, $1\mathrm{e}{-3}$ and $5\mathrm{e}{-4}$; epoch 21-25, $1\mathrm{e}{-4}$ and $5\mathrm{e}{-4}$; epoch 26-30, $5\mathrm{e}{-5}$ and $0$; epoch 31-35, $1\mathrm{e}{-5}$ and $0$; epoch 36-40, $5 \mathrm{e}{-6}$ and $0$; epoch 41-45, $1 \mathrm{e}{-6}$ and $0$. 
%
%AllConCh is optimized using Adam with an initial learning rate $0.0002$ and mini-batch size of $64$ examples for $100$ epochs. 
%
%The dropout ratio for AllConCh, AllConC2 and AllConC3 is $0.25$, for AllConv and AllConC1 is $0$, i.e. \emph{no dropout}.  

%\paragraph{Evaluation Metrics.} We select the model of the least top-1 validation error rate using center-cropped only (Top1c), then evaluate its top-5 error rate with center-cropped only (Top5c), its top-1 error rate averaging over 10 patches (Top1)--center, top right, top left, bottom right, bottom left , together with their horizontal flips, and its top-5 error rate averaging over these 10 patches (Top5), on the validation set. 
%
%We report Top1c, Top5c, Top1 and Top5 results.
%
\begin{figure*}[t]
\centering
\subfigure[conv1]{\includegraphics[width=0.22\textwidth]{figures/CRelu_hist_conv_1-crop.pdf}}\hspace{0.07in}
\subfigure[conv2]{\includegraphics[width=0.22\textwidth]{figures/CRelu_hist_conv_2-crop.pdf}}\hspace{0.07in}
\subfigure[conv3]{\includegraphics[width=0.22\textwidth]{figures/CRelu_hist_conv_3-crop.pdf}}\hspace{0.07in}
\subfigure[conv4]{\includegraphics[width=0.22\textwidth]{figures/CRelu_hist_conv_4-crop.pdf}}
\vspace{-0.15in}
\caption{\textbf{Histograms of $\mu^r$(red) and $\mu^w$(blue) for $\cat$ model on ImageNet.} The two distributions align with each other for all conv1-conv4 layers--as we expected, the pairing phenomenon is not present any more after applying the $\cat$ activation scheme.
}\label{fig:dist_allconc3}
\vspace{-0.25in}
\end{figure*}

The results are provided in Table~\ref{tab:AllConvResult}. 
%
We report the top-1 and top-5 error rates with center crop only and by averaging scores over $10$ patches from the center crop and four corners and with horizontal flip~\cite{krizhevsky2012imagenet}.
%
Interestingly, integrating $\cat$ to conv1-4 achieves the best results, whereas going deeper with higher model capacity does not further benefit the classification performance.
%
In fact, this parallels with our initial observation on AlexNet (Figure~\ref{fig:dist_Alex} in Section~\ref{intuition:conj})---there exists less ``pairing'' in the deeper convolution layers and thus there is not much gain by decomposing the phase in the deeper layers. %the deeper the convolution layer, the less ``pairing''  there is. 
%
$\abs$ networks exhibit the same trend but do not noticeably improve upon the baseline performance, which implies that $\abs$ is not the most suitable candidate for large-scale deep representation learning. 
%
Another interesting observation, which we will discuss further in Section~\ref{sec:invariant}, is that the model integrating $\cat$ into conv1, conv4 and conv7 layers also achieve highly competitive recognition results with even fewer parameters than the baseline model. 
%
%
%In sum, we believe that such an impressive lift of the baseline model by simply modifying the activation scheme is a pleasantly surprising result.\footnote{We note that \citet{springenberg2014striving} reported slightly better result ($41.2\%$ top-1 error rate with center crop only) than our replication result, but still the improvement is significant.}
In sum, we believe that such a significant improvement over the baseline model by simply modifying the activation scheme is a pleasantly surprising result.\footnote{We note that \citet{springenberg2014striving} reported slightly better result ($41.2\%$ top-1 error rate with center crop only) than our replication result, but still the improvement is significant.}
%


%
We also compare our best models with AlexNet and other variants in Table~\ref{tab:ImageNetResult}.
%
Even though reducing the number of parameters is not our primary goal, it is worth noting that our model with only $4.6$M parameters ($\cat$ + all) outperforms FastFood-32-AD (FriedNet)~\cite{yang2014deep} and Pruned AlexNet (PrunedNet)~\cite{han2015learning}, whose designs directly aim at parameter reduction. 
%
Therefore, besides the performance boost, another significance of $\cat$ activation scheme is in designing more parameter-efficient deep neural networks.
%Therefore, besides the performance boost, another significance of $\cat$ activation scheme is in designing more parameter-savvy deep neural networks. % which are crucial in real-world and mobile applications~\cite{chen2015compressing}. 


%\paragraph{Result Summary.}
%First, we compare among our AllConv based models in Table~\ref{tab:AllConvResult}.
%
%Interestingly, integrating $\cat$ to the first few convolution layers achieves the best results, whereas going deeper with higher model capacity does not further benefit the classification performance.
%
%In fact, such phenomenon parallels with our initial observation on AlexNet (Section~\ref{intuition:conj} Figure~\ref{fig:dist_Alex})--the deeper the conv layer, the less ``pairing''  there is. 
%
%Nonetheless, such a notable gain over the baseline model by merely modifying the activation scheme is still a surprising result. 
%
%One feasible explanation is: the lowest layers of a deep CNN is most computationally demanding during training; imposing the disentangling prior through $\cat$, which indeed agrees with the nature of these conv layers, eases the learning. 
%
%On the other hand, the higher conv layers focus on building more semantically abstract and discriminative features for better classification; such disentangling, or information preservation, prior is not as a good fit.
%

%We also compare our best models with AlexNet and its other variants, trained with the same data augmentation procedures, in Table~\ref{ImageNetResult}.
%%
%Even though reducing the number of parameters is not our primary objective, it is worth noting that our AllConCh model with only 4.6 million parameters outperform FastFood-32-AD (FriedNet)~\cite{yang2014deep} and Pruned AlexNet (PrunNet)~\cite{han2015learning}, whose designs directly aim at parameter reduction. 
%%
%Therefore, another potential significance of $\cat$ is to aid in designing more parameter-and-computationally efficient models which are crucial in real-world and mobile applications~\cite{chen2015compressing}. 
 
%
%\begin{table}[h]
%\centering
%\small
%\begin{tabular}{c|c|c|c|c|c} 
%\hline
%Model & top-1 & top-5 & top-1$^*$ & top-5$^*$ & dropout \\ \hline
%Baseline & 41.81 & 19.74  & 38.03  & 17.17  & 0 \\ \hline
%conv1--4 & \textbf{39.82} & \textbf{18.28} & \textbf{36.20}   & \textbf{15.72} & 0 \\ \hline 
%conv1--7 &  39.97 & 18.33 & 36.53 & 16.01& 0.25  \\ \hline
%conv1--9 & 40.15 & 18.58 & 36.50  & 16.14 & 0.25  \\ \hline
%all & 40.93 & 19.39 & 37.28 & 16.72 & 0.25 \\ \hline
%\hline
%\end{tabular}
%\caption{\textbf{Validation error rates on ImageNet dataset.} The best model is AllConC1 where the first 4 conv layers are followed by $\cat$. Adding more $\cat$ does not keep improving the classification results. It is also interesting to note that dropout does not necessarily help in this type of conv architecture.  \label{tab:AllConvResult}}
%\end{table}

==> FeatureLearning.tex <==


\begin{figure*}[t]
\subfigure[Original image]{\includegraphics[width=0.19\textwidth]{figures/staple/test_image1.png}}
%\hspace{0.2in}
\subfigure[conv1]{\includegraphics[width=0.19\textwidth]{figures/staple/output_image1.png}}
%\hspace{0.2in}
\subfigure[conv2]{\includegraphics[width=0.19\textwidth]{figures/staple/output_image2.png}}
%\hspace{0.2in}
\subfigure[conv3]{\includegraphics[width=0.19\textwidth]{figures/staple/output_image3.png}}
%\hspace{0.2in}
\subfigure[conv4]{\includegraphics[width=0.19\textwidth]{figures/staple/output_image4.png}}
%\vspace{2em}
%\centering
%\subfigure[$\relu$ conv1]{\includegraphics[width=0.15\textwidth]{figures/staple_baseline/output_image1.png}}
%\hspace{0.2in}
%\subfigure[$\relu$ conv2]{\includegraphics[width=0.15\textwidth]{figures/staple_baseline/output_image2.png}}
%\hspace{0.2in}
%\subfigure[$\relu$ conv3]{\includegraphics[width=0.15\textwidth]{figures/staple_baseline/output_image3.png}}
%\hspace{0.2in}
%\subfigure[$\relu$ conv4]{\includegraphics[width=0.15\textwidth]{figures/staple_baseline/output_image4.png}}
%\vspace{-2em}
\vspace{-0.05in}
\caption{\textbf{$\cat$ Model Reconstructions.} We use a simple linear reconstruction algorithm (see Algorithm~\ref{Recon_1} in the supplementary materials) to reconstruct the original image from conv1-conv4 features (left to right). The image is best viewed in color/screen.
}\label{fig:recon_1_4}
\vspace{-0.1in}
\end{figure*}

\subsection{Revisiting the Reconstruction Property}\label{sec:feature}
%\subsection{Disentangling Conjecture and Reconstruction Property Revisit}\label{sec:feature}
%
%
%
In Section~\ref{intuition:conj}, we observe that lower layer convolution filters from $\relu$ models form negatively-correlated pairs.  %hypothesize that the standard CNNs disentangle the phase information of an input signal from its modulus information and the filters form pairs.
%
Does the pairing phenomenon still exist for $\cat$ models?
%
%To answer this question, 
We take our best $\cat$ model trained on ImageNet (where the first 4 conv layers are integrated with $\cat$) and repeat the histogram experiments to generate Figure~\ref{fig:dist_allconc3}.
% the same histograms as in Figure~\ref{fig:dist_Alex}
%: take the filters from conv1-conv4 layers where $\relu$ is replaced by $\cat$, calculate the corresponding $\nmu^w_i$ for each layer and plot the histograms of $\nmu^w_i$ along with those of $\nmu^r_i$ for random Gaussian vectors of unit norms in Figure~\ref{fig:dist_allconc3}. 
%
In clear contrast to Figure~\ref{fig:dist_Alex}, the distributions of  $\nmu^w_i$ from $\cat$ model well align with the distributions of $\nmu^r_i$ from random Gaussian filters. 
%these two distributions, both centered close to zero, align with each other for all conv1-conv4 layers--as we expected, the pairing phenomenon is not present any more after applying $\cat$ activation scheme.
%
%In other words, with AlexNet, two filters collaborate to span one single direction, one for the positive phase and the other negative; 
%on the other hand, thanks to $\cat$, one filter represents its unique direction and the model capacity is approximately doubled.
In other words, each lower layer convolution filter now uniquely spans its own direction without a negatively correlated pairing filter, while $\cat$ implicitly plays the role of ``pair-grouping".
%disentangling.   

The empirical gap between $\cat$ and $\abs$ justifies that both modulus and phase information are essential in learning deep CNN features. 
%
In addition, to ensure that the outgoing weights for the positive and negative phase are not merely negations of each other, we measure their correlations for the conv1-7 $\cat$ model trained on ImageNet. 
%
Table~\ref{tab:correlation} compares the averaged correlation between the (normalized) positive-negative-pair (pair) outgoing weights and the (normalized) unmatched-pair (non-pair) outgoing weights.
%
The pair correlations are marginally higher than the non-pair ones but both are on average far below $1$ for all layers. 
%
%This suggests that, contrasting $\abs$, the $\cat$ network does not simply focus on the modulus information but imposes different manipulation over the opposite phases.
This suggests that, in contrast to $\abs$, the $\cat$ network does not simply focus on the modulus information but imposes different manipulation over the opposite phases.
% 

In Section~\ref{sec:recon}, we mathematically characterize the reconstruction property of convolution layers with $\cat$. 
%
Proposition~\ref{recon1} claims that the part of an input spanned by the shifts of the filters can be fully recovered. 
%
ImageNet contains a large number of training images from a wide variety of categories; the convolution filters learned from ImageNet are thus expected to be diverse enough to describe the domain of natural images. 
%produce diverse filters whose superposition almost covers the domain of natural images. 
%
Hence, to qualitatively verify the result from Proposition~\ref{recon1}, we can directly invert features from our best $\cat$ model trained on ImageNet via the simple reconstruction algorithm described in the proof of Proposition~\ref{recon1} (Algorithm~\ref{Recon_1} in the supplementary materials).
%
Figure~\ref{fig:recon_1_4} shows an image from the validation set along with its reconstructions using conv1-conv4 features (see Section~\ref{image_recon} in the supplementary materials for more reconstruction examples).
%
%The goal here is not to design the most fancy reconstruction algorithm, but to qualitatively evaluate our theoretical claim; 
Unlike other reconstruction methods~\cite{dosovitskiy2015inverting,mahendran2014understanding}, our algorithm does not involve any additional learning.
%
Nevertheless, it still produces reasonable reconstructions, which supports our theoretical claim in Proposition~\ref{recon1}. 
%
%

For the convolution layers involving max-pooling operation, it is less straightforward to perform direct reconstruction. 
%
Yet we evaluate the conv+$\cat$+max-pooling reconstruction power via measuring properties of the convolution filters and the details are elaborated in Section~\ref{ReconRatio} of the supplementary materials. 
%Yet we endeavor to evaluate the conv+$\cat$+max-pooling reconstruction power via measuring properties of the convolution filters and the details are elaborated in Section~\ref{ReconRatio} of the supplementary materials. 
%For example, we apply the vanilla linear reconstruction algorithm described in the proof of Proposition~\ref{recon1} on conv1-conv4 features and obtain descent reconstructions (Figure\ref{fig:recon_1_4}).
%
%More reconstruction examples are included in the supplementary material (Section~\ref{image_recon}).
%
%As a conclusion, the conv+$\cat$ layer indeed possesses good reconstruction power, as claimed by Proposition~\ref{recon1}. 
%
%The low coherence constraint on the shifted filters implies that we'd like each learned filter to reflect a fairly distinct direction of the input domain. 
%
%Indeed, the mean of the shifted coherence of the normalized convolutional filters before the first max-pooling from AllConvCatHalf for Cifar-10 and Cifar-100 are $0.037$ and $0.042$ respectively, before the second max-pooling are $0.036$ and $0.048$ respectively, which are small enough to demonstrate that in general shifted distinct filters are quite incoherent. 
%
%These numbers are merely an approximation, which do not directly make Equation (\ref{recon_bound}) a significant bound.
%
%Because there are many other cases where the reconstruction power of the conv+$\cat$+max-pooling is strong yet the low coherence condition does not necessarily need to be satisfied, such as a filter with low frequency, where its shifts are highly coherent with one another and are fairly coherent with other filters' shifts. To sum, with $\cat$, we theoretically and empirically show that the original image can be reconstructed via CNN features to a decent degree.
%

%With the aid of $\cat$ and logical assumptions, we theoretically characterize CNN features' robustness and reconstruction power. 
%
%Together with the abstractness from non-linearity and stacked convolution, CNNs produce high quality features that are generalizable to a variety of vision tasks. 

%Theorem~\ref{recon_error} characterizes the reconstruction property when max-pooling is added after $\cat$, which only applies to CIFAR-10/100 experiments.
%%
%CIFAR images are much less diverse than those from ImageNet.
%%
%Instead of directly inverting features back to the original images, we approximate the $\sqrt{\lambda_{\max}/\tilde{\lambda}_{\min}-1}$ term from Theorem~\ref{recon_error} in Table~\ref{tab:reconstructionratio}.
%%
%More specifically, we take (normalized) conv2 and conv5 filters--the two convolution layers before max-pooling layers--from $\cat$ model with half the number of filters, sample (2000 times) $W_x$ and $\tilde{W}_x$ from the shifts of these filters and calculate the statistics of the resulting $\sqrt{\lambda_{\max}/\tilde{\lambda}_{\min}-1}$; for a qualitative comparison, we perform the same procedures for randomly sampled shifted Gaussian filters of unit norm.
%%
%%
%The term $\sqrt{\lambda_{\max}/\tilde{\lambda}_{\min}} = \sigma_{\max}/\tilde{\sigma}_{\min}$ is approximately the \emph{condition number} $\kappa$ of $W_x$\footnote{Indeed, the sample mean of $\sqrt{\lambda_{\max}/\tilde{\lambda}_{\min}}$ is approximately the same as the sample mean of $\kappa$ for $W_x$.} , which measures the numerical stability of $W_x$, or the geometric distortion under the linear transformation governed by $W_x$.
%%
%In fact, characterizing $\kappa$ for random matrix in the non-asymptotic case--not to mention when shifting is involved--is still a challenging research problem in mathematics~\cite{rudelson2010non}.
%%
%However, our empirical comparison in Table~\ref{tab:reconstructionratio} between learned convolution filters and random Gaussian filters shows that the learned filter matrices generally cause less distortion between input signals and the output features than random filter matrices. 
%%
%More theoretical work in the future along this direction can be valuable\footnote{We provide a simple extension of Theorem~\ref{recon_error} in the supplementary materials, see Corollary~\ref{22extention}}.
%


==> Introduction.tex <==
\section{Introduction}
\label{sec:intro}
%In recent years, convolutional neural networks (CNNs) have achieved great success in many problems of machine learning and computer vision~\cite{krizhevsky2012imagenet,girshick2014rich}. 
In recent years, convolutional neural networks (CNNs) have achieved great success in many problems of machine learning and computer vision~\cite{krizhevsky2012imagenet,simonyan2014very,szegedy2015going,girshick2014rich}.
%
%A wide range of techniques has been researched aiming at enhancing the performance or easing the training of CNNs.
In addition, a wide range of techniques have been developed to enhance the performance or ease the training of CNNs~\cite{lin2013network,zeiler2013stochastic, maas2013rectifier, ioffe2015batch}.
%
%The development of these techniques mostly is through empirical trial-and-error.
%
% Meanwhile, fundamental understanding of CNNs, especially from a theoretical perspective under realistic assumptions, is still lacking. 
% Meanwhile, fundamental understanding of CNNs, especially from a theoretical perspective under realistic assumptions, is still lagging behind. 
%Despite the great empirical success, fundamental understanding of CNNs, especially from a theoretical perspective under realistic assumptions, is still lagging behind. 
Despite the great empirical success, fundamental understanding of CNNs is still lagging behind. 
%
% In this paper, we aim to provide insight on the property of convolutional neural networks, as well as a generic method to improve the performance of many CNN architectures.
Towards addressing this issue, this paper aims to provide insight on the intrinsic property of convolutional neural networks. %, as well as a generic method to improve the performance of many CNN architectures.

%regularization tools such as dropout and dropconnect, optimization methods such as stochastic gradient decent (SGD) and Adam, activation functions such as rectified linear units and maxout, initialization routine such as Xviar, parameter reduction techniques such as Fried and Pruned ConvNet,  
%
%For example, regularization techniques such as dropout and dropconnect  
%Researchers have conducted experiments~\cite{YosinskiCBL14} and built visualization tools~\cite{zeiler2014visualizing} to illustrate the internal operations of these models. 
%
%However, fundamental understanding of CNNs, especially from a theoretical perspective under realistic assumptions, is still lacking. 
%
\begin{figure}
\centering
\includegraphics[width=0.475\textwidth]{figures/alex-synth.pdf}
\caption{\textbf{Visualization of conv1 filters from AlexNet}. Each filter and its pairing filter ($w_i$ and $\bar{w}_i$ next to each other) appear surprisingly opposite (in phase) to each other. See text for details.}\label{fig:CNN_pairs_Alex}
\vspace*{-0.15in}
\end{figure}

\begin{figure*}[htbp]
\centering
\subfigure[conv1]{\includegraphics[width=0.19\textwidth]{figures/Alex_hist_conv_1-crop.pdf}}
\subfigure[conv2]{\includegraphics[width=0.19\textwidth]{figures/Alex_hist_conv_3-crop.pdf}}
\subfigure[conv3]{\includegraphics[width=0.19\textwidth]{figures/Alex_hist_conv_5-crop.pdf}}
\subfigure[conv4]{\includegraphics[width=0.19\textwidth]{figures/Alex_hist_conv_7-crop.pdf}}
\subfigure[conv5]{\includegraphics[width=0.19\textwidth]{figures/Alex_hist_conv_9-crop.pdf}}
\vspace*{-0.15in}
\caption{\textbf{Histograms of $\mu^r$(red) and $\mu^w$(blue) for AlexNet}. 
%
Recall that for a set of unit length filters $\{\phi_i\}$, we define $\mu^{\phi}_i = \langle \phi_i, \bar{\phi}_i  \rangle$ where $\bar{\phi}_i$ is the pairing filter of $\phi_i$.
%
For conv1 layer, the distribution of $\mu^w$ (from the AlexNet filters) is negatively centered, which significantly differs from that of $\mu^r$ (from random filters), whose center is very close to zero. 
%
The center gradually shifts towards zero when going deeper into the network. 
% except for the 5th layer, the more discriminative layer. We conjecture that at layer 5, inputs are already ''in phase'' and well spread out in a smaller subspace. The filters only needs to extract the modulus information, agreeing with Figure~\ref{fig:coherence_dist_VGG}. 
}\label{fig:dist_Alex}
\vspace*{-0.15in}
\end{figure*}
%\cutsubsectionup

%
To better comprehend the internal operations of CNNs, we investigate the well-known AlexNet~\citep{krizhevsky2012imagenet} and thereafter discover that the network learns highly negatively-correlated pairs of filters for the first few convolution layers.
%
Following our preliminary findings, we hypothesize that the lower convolution layers of AlexNet learn redundant filters to extract both positive and negative phase information of an input signal (Section~\ref{intuition:conj}).
 %disentangle the phase information of an input signal from its modulus information 
%
Based on the premise of our conjecture, we propose a novel, simple yet effective activation scheme called \textbf{Concatenated Rectified Linear Unit} ($\cat$).
%
The proposed activation scheme preserves both positive and negative phase information while enforcing non-saturated non-linearity. 
%
The unique nature of $\cat$ allows a mathematical characterization of convolution layers in terms of reconstruction property, which is an important indicator of how expressive and generalizable the corresponding CNN features are (Section~\ref{sec:recon}).
%

In experiments, we evaluate the CNN models with $\cat$ and make a comparison to models with $\relu$ and Absolute Value Rectification Units ($\abs$)~\cite{jarrett2009best} on benchmark object recognition datasets, such as CIFAR-10/100 and ImageNet (Section~\ref{sec:experiments}). 
%
%For a fair assessment of the impact brought by $\cat$, our experiments employ simple architecture and straightforward training procedures. 
%
We demonstrate that simply replacing $\relu$ with $\cat$ for the lower convolution layers of an existing state-of-the-art CNN architecture yields a substantial improvement in classification performance. %, which is not the case with the counterpart $\abs$ models. 
%
% In addition, $\cat$ allows us to attain notable parameter reduction without sacrificing--if not boosting--classification performance when applied appropriately. 
In addition, $\cat$ allows to attain notable parameter reduction without sacrificing classification performance when applied appropriately.
%

We analyze our experimental results from several viewpoints, such as regularization (Section~\ref{sec:regularization}) and invariant representation learning (Section~\ref{sec:invariant}). 
%
Retrospectively, we provide empirical evaluations on the reconstruction property of $\cat$ models; we also confirm that by integrating $\cat$, the original ``pair-grouping" phenomenon vanishes as expected (Section~\ref{sec:feature}). % and that the outgoing weights between positive and negative phase pairs of filters are sufficiently diverse. 
%
%Deviating from the common trial-and-error course, our preliminary findings on the internal operation of existing CNN architectures sparked the idea of $\cat$;
%Deviating from the common trial-and-error course, our preliminary findings on the internal operation of existing CNN architectures sparked the idea of $\cat$;
%
% the follow-up empirical experiments in turn confirmed our initial conjecture as well as brought new insights into the behavior of convolution layers. 
%=======
%Retrospectively, we provided empirical evaluations on the reconstruction property of $\cat$ models; we also confirmed that by integrating $\cat$, the original disentangling phenomenon vanishes as expected (Section~\ref{sec:feature}). 
%
%Deviating from the common trial-and-error course, our preliminary findings on the internal operation of existing CNN architectures sparked the idea of $\cat$;
%
%the follow-up empirical experiments in turn resonated with our initial conjecture and brought new insights into the behavior of convolution layers.  >>>>>>> 9c46e0b0d32520db8ca3cd321e9fa76c34fa5a62
%
% The advancement of our studies conveys the message that by better understanding the nature of CNNs, we are able to reach their higher potential merely with a simple architecture, a smaller number of parameters and a vanilla training procedure. 
Overall, our results suggest that by better understanding the nature of CNNs, we are able to realize their higher potential with a simple modification of the architecture. 
%Our results suggest that better understanding of the properties of the CNNs can lead to significant performance improvement with a simple modification. 

%
%and delve into its theoretical importance in terms of reconstruction property (Section~\ref{sec:recon}).
%  
%\begin{enumerate}
%\item We investigate filters from AlexNet~\citep{krizhevsky2012imagenet} and hypothesize that the first few convolutional layers of AlexNet disentangle the phase information of an input signal from its modulus information (Section~\ref{intuition:conj}).
%%
%\item Inspired by our conjecture, we propose a novel, simple yet effective activation scheme \textbf{Concatenated Rectified Linear Unit} ($\cat$) and delve into its theoretical importance in terms of reconstruction property (Section~\ref{sec:recon}).
%%
%\item We evaluate $\cat$  in comparison to $\relu$ on benchmark object recognition datasets, namely CIFAR-10/100 and ImageNet (Section~\ref{sec:experiments}). 
%%
%\item Lastly, we look at our experimental results from different angles and gain more valuable insight of $\cat$--in particular, its regularization effect  (Section~\ref{sec:regularization}) and its ability to extract more invariant features (Section~\ref{sec:invariant}). 
%\end{enumerate}
%
%
%\begin{figure}[t]
%\centering
%\includegraphics[width=0.45\textwidth]{figures/Alex_learned_pairs_1.png}
%\vspace{-0.05in}
%\caption{\textbf{Visualization of conv1 filters from AlexNet.} Each filter and its ``pairing'' filter ($w_i$ and $\bar{w}_i$ next to each other) are visualized. See Section~\ref{intuition:conj} for more details.}\label{fig:CNN_pairs_Alex}
%\vspace{-0.1in}
%\end{figure}
%
%
%While probing existing classic deep CNN models, we stumble upon interesting discoveries of the conv filters (Section~\ref{intuition:conj}) that sparks the initial idea.
%
%Meanwhile, other works sharing similar spirits also have shed light on the invention of our proposed activation scheme, as highlighted in Section~\ref{intuition:act}.


==> Regularization.tex <==
\cutsubsectionup
\subsection{A View from Regularization}
\label{sec:regularization}
%
In general, a model with more trainable parameters is more prone to overfitting.
%
However, somewhat counter-intuitively, for the all-conv CIFAR experiments, the models with $\cat$ display much less overfitting issue compared to the baseline models with $\relu$, even though it has twice as many parameters (Table~\ref{tab:cifar_results}). 
%
We contemplate that keeping both positive and negative phase information makes the training more challenging, and such effect has been leveraged to better regularize deep networks, especially when working on small datasets.
%
%On the other hand, we can leverage such effect to better regularize deep networks, especially when working on small datasets. 
%
%\subsubsection{Model Complexity Bound}

%
% Not only from empirical evidence, but also, we can describe the regularization effect by deriving a Rademacher complexity bound for the $\cat$ layer followed by linear transformation as follows:
Besides the empirical evidence, we can also describe the regularization effect by deriving a Rademacher complexity bound for the $\cat$ layer followed by linear transformation as follows:
%
\begin{theorem}\label{RCBound}
Let $\mathcal{G}$ be the class of real functions $\R^{\din}\to \R$ with input dimension $\F$, that is, $\mathcal{G} = [\F]_{j=1}^{\din}$. Let $\mathcal{H}$ be a linear transformation function from $\R^{2\din}$ to $\R$, parametrized by $W$, where $\|W\|_2\leq B$. Then, we have
\[\eR (\mathcal{H}\circ \rho_c \circ \mathcal{G}) \leq \sqrt{\din} B \eR (\F).\]
\end{theorem} 
%
%In addition, we derive a bound for the Rademacher complexity of the $\cat$ + linear transformation layer (Theorem~\ref{RCBound}). 
%
%The important result from Theorem~\ref{RCBound} (see Appendix \ref{sec:proof} for proof) is that the complexity bound of $\cat$ + linear transformation is the same as $\relu$ + Linear Transformation as proved in~\citet{wan2013regularization}. 
%
The proof is in Section~\ref{sec:proof_complex} of the supplementary materials. 
%
Theorem~\ref{RCBound} says that the complexity bound of $\cat$ + linear transformation is the same as that of $\relu$ + linear transformation, which is proved by \citet{wan2013regularization}.
%
%In other words, although the number of model parameters increases, doubling the number of input channels for the following convolution layer by $\cat$ does not necessarily increase the model complexity of the networks. 
In other words, although the number of model parameters are doubled by $\cat$, the model complexity does not necessarily increase.
%
% To explore the regularization effects of $\cat$, we compare the Radamacher Complexity of $\cat$ + Linear Transformation $W_c$ and $\relu$ + Linear Transformation $W_r$. 
%
%Denote $\din$ to be the number of input dimension before activation; denote $\dout$ to be the output dimension after Activation + Linear Transformation.  
%
%Assume that the input as well as the output dimension for both cases are the same; also, the layers prior to activation are the same: let $\F$ be a class of real functions, where $\F_j, j = 1 \cdots \din$ corresponds to the input  from previous layer before activation, $\eR(\F)$ is the empirical Rademacher complexity of $\F$. \\
%
%Therefore, $W_r$ is of dimension $\din$ and $W_c$ is of dimension $\din \times 2$. 
%
%Finally, assume that $\|W_r\| \leq B$ and $\|W_c\| \leq B$. 
%
%First, derive the model bound for $\relu$ + $W_r$.
%
%Second derive the model bound for $\cat$ + $W_c$.
%$\mathcal{H}$ be a linear transform function parametrized by $W_c$ 
%\begin{theorem}\label{RCBound}
%Let $\mathcal{G}$ be the class of real functions $\R^{2\din}\to \R$ with input dimension $2\F$, that is, $\mathcal{G} = [\F]_{j=1}^{2\din}$. Let $\mathcal{H}$ be a linear transform function from $\R^{2\din}$ to $\R$, parametrized by $W$, where $\|W\|_2\leq B$. Then $\eR (\mathcal{H}\circ \rho_c \circ \mathcal{G}) \leq \sqrt{\din} B \eR (\F)$.
%\end{theorem} 


==> RelatedWork.tex <==
\section{Related Works}
\label{sec:relatedworks}



==> theory.tex <==
\cutsectionup
\section{CRelu and Reconstruction Property}
\subsection{Conjecture on Convolution Layers}\label{intuition:conj}
In our initial exploration of classic CNNs trained on natural images such as AlexNet~\cite{krizhevsky2012imagenet}, we noted a curious property of the first convolution layer filters: \emph{these filters tend to form ``pairs''}. % (i.e., two filters with opposite phase).
%During our initial exploration of classic CNNs trained on natural images such as AlexNet~\cite{krizhevsky2012imagenet}, we have noted a curious tendency of the first convolution layer filters: \emph{these filters tend to form ``pairs''}. % (i.e., two filters with opposite phase).
%
More precisely, assuming unit length vector for each filter $\phi_{i}$, we define a \emph{pairing filter} of $\phi_{i}$ in the following way:
$\bar{\phi}_i = \argmin_{\phi_j} \langle \phi_i,\phi_j \rangle.$
%
We also define their cosine similarity $\mu^{\phi}_i = \langle \phi_i, \bar{\phi}_i  \rangle$.
%
%Next, we take the AlexNet~\cite{krizhevsky2012imagenet} trained on ImageNet~\cite{deng2009imagenet} as an example. 
%

%In Figure~\ref{fig:CNN_pairs_Alex}, we match each (normalized) conv1 filter $w_i$ from AlexNet with its pairing filter, and we find that they appear surprisingly opposite to each other, i.e.\ for each $w_i$, there does exist another filter that is almost on the opposite phase.
%
In Figure~\ref{fig:CNN_pairs_Alex}, we show each normalized filter of the first convolution layer from AlexNet with its pairing filter. 
%
Interestingly, they appear surprisingly opposite to each other, i.e., for each filter, there does exist another filter that is almost on the opposite phase.
%
Indeed, AlexNet employs the popular non-saturated activation function, \emph{Rectified Linear Unit} ($\relu$)~\cite{nair2010rectified}, which zeros out negative values and produces sparse activation. 
%
As a consequence, if both the positive phase and negative phase along a specific direction participate in representing the input space, the network then needs to learn two linearly dependent filters of both phases. 

%
To systematically study the pairing phenomenon in higher layers, we graph the histograms of $\nmu^w_i$'s for conv1-conv5 filters from AlexNet in Figure~\ref{fig:dist_Alex}.
%
% We also sample random Gaussian filters of unit norm and plot the histograms of the corresponding $\nmu^r_i$'s to compare. 
For comparison, we generate random Gaussian filters $r_{i}$'s of unit norm\footnote{We sample each entry from standard normal distribution independently and normalize the vector to have unit $l^2$ norm.} and plot the histograms of $\nmu^r_i$'s together.
%
For conv1 layer, we observe that the distribution of $\nmu^w_i$ is negatively centered; by contrast, the mean of $\nmu^r_i$ is only slightly negative with a small standard deviation.
%
Then the center of $\nmu^w_i$ shifts towards zero gradually when going deeper into the network.
%
This implies that convolution filters of the lower layers tend to be paired up with one or a few others that represent their opposite phase, while the phenomenon gradually lessens as they go deeper.
%
%However, such pairing phenomenon gradually lessens while the depth of the convolution layers increases. 

%
Following these observations, we hypothesize that despite $\relu$ erasing negative linear responses, \emph{the first few convolution layers of a deep CNN manage to capture both negative and positive phase information through learning pairs or groups of negatively correlated filters}.
%
This conjecture implies that there exists a redundancy among the filters from the lower convolution layers. 

In fact, for a very special class of deep architecture, the invariant scattering convolutional network~\cite{bruna2013invariant}, it is well-known that its set of convolution filters, which are wavelets, is overcomplete in order to be able to fully recover the original input signals.
%
On the one hand, similar to $\relu$, each individual activation within the scattering network preserves partial information of the input.
%
On the other hand, different from $\relu$ but more similar to $\abs$, scattering network activation preserves the energy information, i.e., keeping the modulus of the responses but erasing the phase information; $\relu$ from a generic CNN, as a matter of fact, retains the phase information but eliminates the modulus information when the phase of a response is negative. 
%
% In addition, while the wavelets for scattering networks are manually engineered, convolution filters from CNNs must be learned, which challenges any rigorous theoretical justification. 
In addition, while the wavelets for scattering networks are manually engineered, convolution filters from CNNs must be learned, which makes the rigorous theoretical analysis challenging.  
%In other words, in order for a filter to be activated, it not only needs to be closely aligned with a major direction constituting the input signal but also in the same phase.
%
%This type of non-negative representation is consistent with the biological model of neuron firing~\cite{lin2011functional}.
%
%In practice, the phase information is also substantial to certain machine learning tasks in computer vision~\cite{coates2011importance,poultney2006efficient}. 
%

%
%
%Suppose we can leverage the pairing prior and design a simple scheme to explicitly allow both positive and negative activation, we will be able to alleviate such redundancy and make more efficient use of the trainable parameters.
Now suppose we can leverage the pairing prior and design a method to explicitly allow both positive and negative activation, then we will be able to alleviate the redundancy among convolution filters caused by $\relu$ non-linearity and make more efficient use of the trainable parameters.
%
To this end, we propose a novel activation scheme, \emph{Concatenated Rectified Linear Units}, or $\cat$.
%
It simply makes an identical copy of the linear responses after convolution, negate them, concatenate both parts of activation, and then apply $\relu$ altogether. 
%
More precisely, we denote $\relu$ as $[\cdot]_+ \triangleq  \max(\cdot, 0)$, and define $\cat$ as follows:
%
\begin{Definition}\label{crelu}
$\cat$ activation, denoted by $\rho_c: \R \to \R^2$, is defined as follows: $\forall x\in \R, \rho_c(x) \triangleq ([x]_+, [-x]_+)$.  
\end{Definition}
\cutsectiondown
%
%The core spirit of our activation scheme is to allow a filter to be activated in both positive and negative direction while maintaining the same degree of non-saturated non-linearity.
The rationale of our activation scheme is to allow a filter to be activated in both positive and negative direction while maintaining the same degree of non-saturated non-linearity.

%
%
%\subsection{Related Activation Functions}\label{intuition:act} 
%The most popular non-saturated activation function is \emph{rectified linear unit} ($\relu$)~\cite{nair2010rectified}, which zeros out any negative part and produces sparse activation. 
%
%Despite the common belief that sparsity benefits deep neural nets, empirical studies show that it is not always the case.
%
An alternative way to allow negative activation is to employ the broader class of non-saturated activation functions including Leaky $\relu$ and its variants~\cite{maas2013rectifier,xu2015empirical}. 
%Recently, a broader class of non-saturated activation functions, namely Leaky $\relu$ and its variants, are being investigated by practitioners~\cite{xu2015empirical}. 
%
Leaky $\relu$ assigns a small slope to the negative part instead of completely dropping it.  
%
%These activation functions share similar spirits with $\cat$ in the sense that they both tackle the two potential problems caused by the hard $0$ activation: the weights of a filter will not be adjusted if it is never activated; eliminating all negative information can inhibit the learning.
These activation functions share similar motivation with $\cat$ in the sense that they both tackle the two potential problems caused by the hard zero thresholding: (1) the weights of a filter will not be adjusted if it is never activated, and (2) truncating all negative information can potentially hamper the learning.
%
However, $\cat$ is based on an activation \emph{scheme} rather than a \emph{function}, which fundamentally differentiates itself from Leaky $\relu$ or other variants.
%
In our version, we apply $\relu$ after separating the negative and positive part to compose $\cat$, but it is not the only feasible non-linearity. 
%
% If interested, one may experiment combining $\cat$ with other activation functions, such as Leaky $\relu$, to add more diversity to the architecture (possibly on top of additional tuning). 
For example, $\cat$ can be combined with other activation functions, such as Leaky $\relu$, to add more diversity to the architecture. 
%Moreover, researchers have shown that CNN features trained on large, diverse datasets possess reconstruction power and can be generalized to unseen datasets: \citet{mahendran2014understanding} invert CNN features back to the input images under simple natural image priors; \citet{donahue2013decaf} repurpose CNN features trained on ImageNet to novel generic tasks and achieve state-of-the-art results.  
%%
%Therefore, eliminating all negative information to create non-linearity for the lower conv layers could have abandoned too much information.
%%
%Inspired by Section~\ref{intuition:conj} and~\ref{intuition:act}, we would like to design a new activation scheme that reflects the disentangling prior, engages non-saturated activation and treats the positive part and negative part in an equal manner. 
%

Another natural analogy to draw is between $\cat$ and $\abs$, where the latter one only preserves the modulus information but discard the phase information, similar to the scattering network. 
%
$\abs$ has not been widely used recently for the CNN models due to its suboptimal empirical performance.
%
We confirm this common belief in the matter of large-scale image recognition task (Section~\ref{sec:experiments}) and conclude that modulus information alone does not suffice to produce state-of-the-art deep CNN features. 
\subsection{Reconstruction Property}\label{sec:recon}
%Moreover, researchers have shown that CNN features trained on large, diverse datasets possess reconstruction power and can be generalized to unseen datasets: \citet{mahendran2014understanding} invert CNN features back to the input images under simple natural image priors; \citet{donahue2013decaf} repurpose CNN features trained on ImageNet to novel generic tasks and achieve state-of-the-art results.  
%%
%Therefore, eliminating all negative information to create non-linearity for the lower conv layers could have abandoned too much information.
%%
A notable property of $\cat$ is its \emph{information preservation nature}: $\cat$ conserves both negative and positive linear responses after convolution.
%
A direct consequence of information preserving is the reconstruction power of the convolution layers equipped with $\cat$. 
% Such an information preservation nature intuitively links to the reconstruction property of the corresponding networks.
% 

%Reconstruction property of a CNN signifies that its features are expressive and transferable~\cite{YosinskiCBL14}.
Reconstruction property of a CNN implies that its features are representative of the input data.
%
%Researchers have shown great interest in this aspect of CNNs: \citet{mahendran2014understanding} invert CNN features back to the input under simple natural image priors; \citet{zhao2015stacked} stack autoencoders with reconstruction objective to build better classifiers. %\citet{donahue2013decaf} repurpose CNN features trained on ImageNet to novel generic tasks and achieve state-of-the-art results.
This aspect of CNNs has gained interest recently: \citet{mahendran2014understanding} invert CNN features back to the input under simple natural image priors; \citet{zhao2015stacked} stack autoencoders with reconstruction objective to build better classifiers. %\citet{donahue2013decaf} repurpose CNN features trained on ImageNet to novel generic tasks and achieve state-of-the-art results.
%
%Theorists also have attempted to analytically characterize such property of CNNs. 
%
\citet{bruna2013signal} theoretically investigate general conditions under which the max-pooling layer followed by $\relu$ is injective and measure stability of the inverting process by computing the Lipschitz lower bound.
%
However, their bounds are non-trivial only when the number of filters significantly outnumbers the input dimension, which is not realistic. 
%
%Indeed, besides max-pooling erasing the location information, the rectifier operator, $\relu$, also poses a challenge for such analysis by eliminating all negative activations. 
%

In our case, it becomes more straightforward to analyze the reconstruction property since $\cat$ preserves all the information after convolution.
%
The rest of this section mathematically characterizes the reconstruction property of a single convolution layer followed by $\cat$ with or without max-pooling layer.
%, deliberately separates the positive and negative phases and applies a simple absolute value function as nonlinearity at the end.   
%
%Therefore, 
%


%

%\paragraph{Convolution + $\cat$.}
%
We first analyze the reconstruction property of convolution followed by $\cat$ without max-pooling.
%
This case is directly pertinent as deep networks replacing max-pooling with stride has become more prominent in recent studies~\cite{springenberg2014striving}.
%
The following proposition states that the part of an input signal spanned by the shifts of the filters is well preserved.
%Deep networks replacing max-pooling with stride 2 convolution has become more prominent in recent studies. 
%
%Hence this case is directly pertinent.
%
%In fact, for our ImageNet experiments (see Section~\ref{sec:exp-imagenet}), there is no max-pooling layer; hence this case is directly relevant.
%
%Hence, this case is directly relevant.  
%
\begin{proposition}\label{recon1}
Let $x\in\mathbb{R}^{D}$ be an input vector\footnote{For clarity, we assume the input signals are vectors (1D) rather than images (2D); however, similar analysis can be done for 2D case.} and $W$ be the $D$-by-$K$ matrix whose columns vectors are composed of $w_i \in\mathbb{R}^l, i = 1, \ldots ,K$ convolution filters. Furthermore, let $x = x' +  (x - x')$, where $x' \in\mathrm{range}(W)$ and $x-x' \in \mathrm{ker}(W)$. Then we can reconstruct $x'$ with $\cnn(x)$, where $\cnn(x)\triangleq \cat\left(W^{T}x\right)$.
\end{proposition}
%
See Section~\ref{nonmax} in the supplementary materials for proof.
%Proposition~\ref{recon1} (see Section~\ref{nonmax} in the supplementary materials for proof) states that the part of an input signal spanned by the shifts of the filters is well preserved.
% and can be reconstructed via a simple linear algorithm.
%

%
Next, we add max-pooling into the picture.
%
To reach a non-trivial bound, we need additional constraints on the input space.
%
Due to space limit, we carefully explain the constraints and the theoretical consequence in Section~\ref{maxpooling} of the supplementary materials. 
%
We will revisit this subject after the experiment section (Section~\ref{sec:feature}). %from an empirical point of view. 
